DerivKit: stable numerical derivatives bridging Fisher forecasts and MCMC

DerivKit is a Python package for derivative-based statistical inference. It implements stable numerical differentiation and derivative assembly utilities for Fisher-matrix forecasting and higher-order likelihood approximations in scientific applications, supporting scalar- and vector-valued models including black-box or tabulated functions where automatic differentiation is impractical or unavailable. These derivatives are used to construct Fisher forecasts, Fisher bias estimates, and non-Gaussian likelihood expansions based on the Derivative Approximation for Likelihoods (DALI). By extending derivative-based inference beyond the Gaussian approximation, DerivKit forms a practical bridge between fast Fisher forecasts and more computationally intensive sampling-based methods such as Markov chain Monte Carlo (MCMC).

==> sections/api.tex <==
\subsection{Example Usage}
\label{subsec:api_example_usage}

The package is structured into modules for finite differences, adaptive fits, diagnostics, plotting, and DALI utilities.
A minimal, typed API is provided together with tests and usage examples in notebooks.


The following snippet demonstrates how to estimate the second derivative of \( f(x) = x^2 \) at \( x = 0.5 \) using \pkg{DerivKit}'s adaptive and finite-difference methods, and compares them to \pkg{numdifftools}:

\noindent\rule{\linewidth}{0.4pt}  % Top horizontal line

\begin{verbatim}
1 from derivkit.kit import DerivativeKit  # import main module
2 import numdifftools as nd  # for reference
3 
4 def func(x):  # test function
5     return x**2
6 
7 order = 2 # 2nd derivative
8 x0 = 0.5 # evaluation point
9 true_val = 2.0 # analytical value
10 
11 dk = DerivativeKit(func, x0, derivative_order=order)  # init
12 
13 stencil_val = dk.finite.compute()  # 5-point stencil
14 adaptive_val = dk.adaptive.compute()  # adaptive poly fit
15 nd_val = nd.Derivative(f, n=order)(x0)  # numdifftools reference
16 
17 err_abs_stencil = abs(stencil_val - true_val)
18 err_abs_adaptive = abs(adaptive_val - true_val)
19 
20 print(f"Deriv order {order} of f(x)=x² at x={x0}")
21 print(f"True:     {true_val:.4f}")
22 print(f"Stencil:  {stencil_val:.4f} (err: {err_abs_stencil:.1e})")
23 print(f"Adaptive: {adaptive_val:.4f} (err: {err_abs_adaptive:.1e})")
24 print(f"NumDiff:  {nd_val:.4f}")
\end{verbatim}

\noindent\rule{\linewidth}{0.4pt} 

\vspace{0.5em}


This simple test confirms that both derivative estimators in \pkg{DerivKit} match the expected value, validating correctness in a controlled setting.

\noindent
In cosmological applications, the target function is often a data vector, such as angular power spectra $C_\ell$, evaluated as a function of cosmological parameters.
The snippet below illustrates how to compute the derivative of such a vector-valued function with respect to \texttt{Omega\_m}:

\noindent\rule{\linewidth}{0.4pt}
\begin{verbatim}
 1 # Compute the derivative of a vector-valued observable (Cls)
 2 # with respect to Omega_m
 3 def cls_omega_m(omega_m):
 4     params = fiducial.copy()
 5     params["omega_m"] = omega_m
 6     # vector-valued output
 7     # (e.g. shape: flattened [n_ells * n_corr])
 8     # implementation of compute_cls(params) depends on your setup
 9     return compute_cls(params)   
10 
11 # Derivative at fiducial value
12 dk = DerivativeKit(
13     cls_omega_m,
14     central_value=omega_m,
15     derivative_order=1
16 )
17 ddatavec_domegam = dk.adaptive.compute()  # returns vector derivative
\end{verbatim}

\noindent\rule{\linewidth}{0.4pt} 

\noindent
For matrix-shaped outputs (\eg, \texttt{[n\_ells, n\_corr]}), simply flatten the result in the function using \texttt{.flatten()} before returning it.

==> sections/validation.tex <==
\section{Validation and results}
We validate on functions with known derivatives (polynomials, $\sin$, $\exp$) and noisy settings, comparing error scaling against standard finite differences \citep{Fornberg:1998,Lyness:1976} \niko{missing refs, add to bib - - was this mine? lol }. 
We further show that doublet-DALI expansions built from \texttt{DerivKit} track the true likelihood on a representative toy model (although, as shown in \citep{Ryan:2022qpa}, doublet-DALI provides a poor approximation to the posterior when the parameter dependence is sublinear), thus enabling substantial speedups relative to full MCMC chains.

\input{figures/dali_demo}

